Single event effects in the HCCStar ASICs for ITk strip upgrade

Triple Modular Redundancy (TMR) technology has been implemented in the design of the HCCStar to reduce digital state changes and ensure reliable operation. We tested the effectiveness of the protection by placing HCCStar chips in a proton beam. We studied corrected bit flips in registers and actual single event effects in the LCB and LP paths under different proton energies. Our estimate is that the LP data-loss fraction relative to the 400 kHz readout is $O(10^{-10})$ during normal operation and there will be $O(10)$ corrected bit flips per HCCStar bit per year at the HL-LHC.

==> Makefile <==
# Makefile for creating an ATLAS LaTeX document

# Copyright (C) 2002-2025 CERN for the benefit of the ATLAS collaboration
#------------------------------------------------------------------------------
# By default makes ANA-BPHY-2025-04-INT1.pdf using target run_pdflatex.
# Replace ANA-BPHY-2025-04-INT1 with your main filename or add another target set.
# Replace BIBTEX = biber with BIBTEX = bibtex if you use bibtex instead of biber.
# Adjust FIGSDIR for your figures directory tree.
# Adjust the %.pdf dependencies according to your directory structure.
# Use "make clean" to cleanup.
# Use "make cleanpdf" to delete $(BASENAME).pdf.
# "make cleanall" also deletes the PDF file $(BASENAME).pdf.
# Use "make cleanepstopdf" to remove PDF files created automatically from EPS files.
#   Note that FIGSDIR has to be set properly for this to work.

# Set the default target to run_pdflatex instead of run_latexmk to use explicit
# pdflatex/biber commands to compile.

# You can use the target version to check your TeX Live version.

#-------------------------------------------------------------------------------
# Check which TeX Live installation you have with the command pdflatex --version
PDFLATEX = pdflatex
# BIBTEX   = bibtex
BIBTEX   = biber
# TLVERS   = $(shell pdflatex --version | grep -Go 'TeX Live [0-9]*' | grep -Go '[0-9].*')
# TWIKI    = https://twiki.cern.ch/twiki/bin/view/AtlasProtected/PubComLaTeXFAQ

#-------------------------------------------------------------------------------
# The main document filename
BASENAME = main

#-------------------------------------------------------------------------------
# Adjust this according to your top-level figures directory
# This directory tree is used by the "make cleanepstopdf" command
FIGSDIR  = figs
#-------------------------------------------------------------------------------

# EPSTOPDFFILES = `find . -name \*eps-converted-to.pdf`
rwildcard=$(foreach d,$(wildcard $1*),$(call rwildcard,$d/,$2) $(filter $(subst *,%,$2),$d))
EPSTOPDFFILES = $(call rwildcard, $(FIGSDIR), *eps-converted-to.pdf)

# Default target - make ANA-BPHY-2025-04-INT1.pdf with latexmk.
default: run_latexmk
# Use pdflatex/biber instead to compile.
# default: run_pdflatex

.PHONY: run_latexmk
.PHONY: newdocument newdocumenttexmf newnotemetadata newpapermetadata newfiles
.PHONY: draftcover preprintcover newdata
.PHONY: version clean cleanpdf help

# Check TeX Live version
# version:
# 	@echo "Checking version"
# 	@echo "TLVERS $(TLVERS), TEXLIVE $(TEXLIVE)"
# 	@if [ $(TLVERS) -lt $(TEXLIVE) ]; then \
# 		echo "Your TeX Live version ($(TLVERS)) is older than $(TEXLIVE). Please consult $(TWIKI)"; \
# 	fi

# Standard pdflatex target
run_pdflatex: $(BASENAME).pdf
	@echo "Made $<"

# Remove -pdf option to run latex instead of pdflatex
run_latexmk:
	latexmk -pdf $(BASENAME)

#-------------------------------------------------------------------------------
# Specify the tex and bib file dependencies for running pdflatex
# If your bib files are not in the main directory adjust this target accordingly
#%.pdf: %.tex *.tex bib/*.bib
%.pdf:  %.tex *.tex *.bib
	$(PDFLATEX) $<
	-$(BIBTEX)  $(basename $<)
	$(PDFLATEX) $<
	$(PDFLATEX) $<
#-------------------------------------------------------------------------------

# Default is to make a new paper
new: newnote

newpaper: TEMPLATE=atlas-paper
newpaper: newdocument newfiles newpapermetadata newauxmat

newpapertexmf: TEMPLATE=atlas-paper
newpapertexmf: newdocumenttexmf newfiles newpapermetadata newauxmat

newnote: TEMPLATE=atlas-note
newnote: newdocument newfiles newnotemetadata

newnotetexmf: TEMPLATE=atlas-note
newnotetexmf: newdocumenttexmf newfiles newnotemetadata

newbook: TEMPLATE=atlas-book
newbook: newdocument newfiles newpapermetadata

newbooktexmf: TEMPLATE=atlas-book
newbooktexmf: newdocumenttexmf newfiles newpapermetadata

draftcover:
	cp  template/atlas-draft-cover.tex $(BASENAME)-draft-cover.tex

preprintcover:
	cp template/atlas-preprint-cover.tex $(BASENAME)-preprint-cover.tex

newdata:
	sed s/atlas-document/$(BASENAME)/ template/atlas-hepdata-main.tex >$(BASENAME)-hepdata-main.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

newdocument:
	sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex >$(BASENAME).tex

newdocumenttexmf:
	sed s/atlas-document/$(BASENAME)/ template/$(TEMPLATE).tex | \
	sed 's/\\RequirePackage{latex\/atlaslatexpath}/% \\RequirePackage{latex\/atlaslatexpath}/' \
	>$(BASENAME).tex

newpapermetadata:
	cp template/atlas-paper-metadata.tex $(BASENAME)-metadata.tex

newnotemetadata:
	cp template/atlas-note-metadata.tex $(BASENAME)-metadata.tex

newfiles:
	echo "% Put you own bibliography entries in this file" > $(BASENAME).bib
	touch $(BASENAME)-defs.sty

newauxmat:
	cp template/atlas-auxmat.tex $(BASENAME)-auxmat.tex
	cp template/atlas-hepdata.tex $(BASENAME)-hepdata.tex

help:
	@echo "To create a new paper/CONF Note/PUB Note draft give the command:"
	@echo "make newpaper [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo "To create a new ATLAS note draft give the command:"
	@echo "make newnote [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo "To create a long document (book) like a TDR:"
	@echo "make newbook [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo ""
	@echo "To compile the paper give the command"
	@echo "make"
	@echo "If your bib files are not in the main directory, adjust the %.pdf target accordingly."
	@echo ""
	@echo "To compile the document using latexmk give the command:"
	@echo "make run_latexmk"
	@echo "You can also adjust the 'default' target."
	@echo ""
	@echo "If atlaslatex is installed centrally, e.g. in ~/texmf:"
	@echo "make newpapertexmf|newnotetexmf|newbooktemf [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo ""
	@echo "If you need a standalone draft cover give the commands:"
	@echo "make draftcover [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo "pdflatex ANA-BPHY-2025-04-INT1-draft-cover"
	@echo ""
	@echo "If you need a standalone preprint cover give the commands:"
	@echo "make preprintcover [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo "pdflatex ANA-BPHY-2025-04-INT1-preprint-cover"
	@echo ""
	@echo "If you need a document for HepData material give the commands:"
	@echo "make newdata [BASENAME=ANA-BPHY-2025-04-INT1]"
	@echo "pdflatex ANA-BPHY-2025-04-INT1-hepdata-main"
	@echo ""
	@echo "make clean    to clean auxiliary files (not output PDF)"
	@echo "make cleanpdf to clean output PDF files"
	@echo "make cleanall to clean all files"
	@echo "make cleanepstopdf to clean PDF files automatically made from EPS"
	@echo ""

clean:
	-rm *.toc *.aux *.lof *.lot *.log *.out \
		*.bbl *.blg *.brf *.bcf *-blx.bib *.run.xml \
		*.cb *.ind *.idx *.ilg *.inx *.tdo \
		*.synctex.gz *-SAVE-ERROR *~ *.fls *.fdb_latexmk .*.lb spellTmp

cleanpdf:
	-rm $(BASENAME).pdf
	-rm $(BASENAME)-draft-cover.pdf $(BASENAME)-preprint-cover.pdf
	-rm $(BASENAME)-hepdata-main.pdf

cleanall: clean cleanpdf

# Clean the PDF files created automatically from EPS files
cleanepstopdf: $(EPSTOPDFFILES)
	@echo "Removing PDF files made automatically from EPS files"
	-rm $^

